Entity Matching using Large Language Models

Entity matching is the task of deciding whether two entity descriptions refer to the same real-world entity. Entity matching is a central step in most data integration pipelines. Many state-of-the-art entity matching methods rely on pre-trained language models (PLMs) such as BERT or RoBERTa. Two major drawbacks of these models for entity matching are that (i) the models require significant amounts of task-specific training data and (ii) the fine-tuned models are not robust concerning out-of-distribution entities. This paper investigates using generative large language models (LLMs) as a less task-specific training data-dependent and more robust alternative to PLM-based matchers. The study covers hosted and open-source LLMs which can be run locally. We evaluate these models in a zero-shot scenario and a scenario where task-specific training data is available. We compare different prompt designs and the prompt sensitivity of the models. We show that there is no single best prompt but that the prompt needs to be tuned for each model/dataset combination. We further investigate (i) the selection of in-context demonstrations, (ii) the generation of matching rules, as well as (iii) fine-tuning LLMs using the same pool of training data. Our experiments show that the best LLMs require no or only a few training examples to perform comparably to PLMs that were fine-tuned using thousands of examples. LLM-based matchers further exhibit higher robustness to unseen entities. We show that GPT4 can generate structured explanations for matching decisions and can automatically identify potential causes of matching errors by analyzing explanations of wrong decisions. We demonstrate that the model can generate meaningful textual descriptions of the identified error classes, which can help data engineers to improve entity matching pipelines.

==> figures/cc_explanation_examples.tex <==
\begin{figure}[]
\centering
\includegraphics[width=\linewidth]{figures/data/cc_explanation_examples.png}
\caption{Two corner-case examples predicted as non-match and their explanations. The upper example is a false negative, the lower a true negative.} \label{fig:cc-explanation-example}
\end{figure}

==> figures/roc_curve.tex <==
\begin{figure}[]
\centering
\includegraphics[width=\linewidth]{figures/data/roc-curve.png}
\caption{ROC-curves generated with LLM supplied confidence values.} \label{fig:summarization-prompt}
\end{figure}

==> tables/confidence-comparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Comparison of GPT4-generated confidence scores and their correlation with the correct decision. Correlation is calculated using Pearsons Correlation Coefficient.}
\label{tab:confidence-comparison}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}l|c|c|c@{}}
\toprule
 &
  \begin{tabular}[c]{@{}c@{}}Mean Confidence\\ (correct decision)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Mean Confidence\\ (wrong decision)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Correlation Confidence\\ with Correctness\end{tabular} \\ \midrule
Walmart-Amazon & 88.73 & 86.10 & 13.64 \\
DBLP-Scholar   & 93.81 & 88.85 & 16.64 \\
WDC Products   & 95.84 & 89.52 & 26.47 \\ \bottomrule
\end{tabular}%
}
\end{table}

==> tables/error-classes-dblp_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Generated error classes for the DBLP-Scholar dataset and manually annotated number of errors.}
\label{tab:error-classes-dblp}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lc@{}}
\toprule
\multicolumn{1}{c}{False Negatives (26 overall)} &
  \# errors \\ \midrule
\begin{tabular}[c]{@{}l@{}}\textbf{1. Year Discrepancy:} Differences in publication years lead to false negatives,\\ even when other attributes match closely.\end{tabular} &
  8 \\
\begin{tabular}[c]{@{}l@{}}\textbf{2. Venue Variability:} Variations in how the publication venue is listed (e.g., \\ abbreviations, full names) cause mismatches.\end{tabular} &
  14 \\
\begin{tabular}[c]{@{}l@{}}\textbf{3. Author Name Variations:} Differences in author names, including initials, \\ order of names, or inclusion of middle names, lead to false negatives.\end{tabular} &
  9 \\
\begin{tabular}[c]{@{}l@{}}\textbf{4. Title Variations:} Minor differences in titles, such as missing words or \\ different word order, can cause false negatives.\end{tabular} &
  11 \\
\begin{tabular}[c]{@{}l@{}}\textbf{5. Author List Incompleteness:} Differences in the completeness of the author \\ list, where one entry has more authors listed than the other.\end{tabular} &
  11 \\ \midrule
\multicolumn{1}{c}{False Positives (26 overall)} &
  \# errors \\ \midrule
\begin{tabular}[c]{@{}l@{}}\textbf{1. Overemphasis on Title Similarity:} High similarity in titles leading to false\\ positives, despite differences in other critical attributes.\end{tabular} &
  15 \\
\begin{tabular}[c]{@{}l@{}}\textbf{2. Author Name Similarity Overreach:} False positives due to high similarity\\ in author names, ignoring discrepancies in other attributes.\end{tabular} &
  16 \\
\begin{tabular}[c]{@{}l@{}}\textbf{3. Year and Venue Ignored:} Cases where the year and venue match or are\\ close, but other discrepancies are overlooked.\end{tabular} &
  5 \\
\begin{tabular}[c]{@{}l@{}}\textbf{4. Partial Information Match:} Matching based on partial information, such\\ as incomplete author lists or titles, leading to false positives.\end{tabular} &
  19 \\
\begin{tabular}[c]{@{}l@{}}\textbf{5. Misinterpretation of Publication Types:} Confusing different types of\\ publications (e.g., conference vs. journal) when other attributes match.\end{tabular} &
  9 \\ \bottomrule
\end{tabular}%
}
\end{table}

==> tables/finetuning_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[]
\centering
\caption{Results for fine-tuning Turbo06 and transfer to all datasets. Left-most column shows the dataset used for fine-tuning. Best result is bold, second best is underlined.}
\label{tab:fine-tuning}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule
                  & WDC                          & A-B                          & W-A                         & A-G                         & D-S                         & D-A                         \\ \midrule
WDC Products      & {\ul 88.34}                  & {\ul 94.69}                  & {\ul 90.55}                 & 77.82                       & 88.97                       & 95.60                       \\
Abt-Buy           & 62.53                        & 94.18                        & 90.19                       & {\ul 79.84}                 & 89.36                       & 96.15                       \\
Walmart-Amazon    & 52.33                        & 92.80                        & \textbf{92.76}              & 78.80                       & 87.93                       & 97.42                       \\
Amazon-Google     & 48.66                        & 89.97                        & 87.26                       & 79.81                       & 91.01                       & 96.15                       \\
DBLP-Scholar      & 11.32                        & 57.24                        & 57.55                       & 35.33                       & \textbf{92.49}              & 98.02                       \\
DBLP-ACM          & 20.00                        & 79.20                        & 65.37                       & 42.46                       & 88.93                       & \textbf{99.40}              \\ \midrule
Best ZS Turbo06   & 74.96                        & 83.83                        & 69.12                       & 63.50                       & 83.04                       & 95.11                       \\
Best FS/R Turbo06 & 80.93                        & 93.14                        & 80.27                       & \textbf{82.58}              & 82.92                       & 97.83                       \\
Best ZS GPT4      & \textbf{89.61}               & \textbf{95.78}               & 89.67                       & 76.38                       & 89.82                       & 98.41                       \\
$\Delta$ GPT4/FT  & {\color[HTML]{FE0000} -1.27} & {\color[HTML]{FE0000} -1.09} & {\color[HTML]{6434FC} 3.09} & {\color[HTML]{6434FC} 3.46} & {\color[HTML]{6434FC} 2.67} & {\color[HTML]{6434FC} 0.99} \\ \bottomrule
\end{tabular}%
}
\end{table}

==> tables/similarity-comparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Comparison of GPT4-generated similarity scores with Cosine and Generalized Jaccard similarity both on the full strings and solely attributes used in the explanations. Number in brackets shows correlation with GPT4 value calculated with Pearsons Correlation Coefficient.}
\label{tab:similarity-comparison}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}l|ccc|ccc|c@{}}
\toprule
 &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Mean Similarities\\ (full string)\end{tabular}} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Mean Similarities\\ (extracted attributes)\end{tabular}} &
   \\ \midrule
 &
  GPT4 &
  Cosine &
  GenJac &
  GPT4 &
  Cosine &
  GenJac &
  \begin{tabular}[c]{@{}c@{}}Mean overlap full string \\ and extracted attributes\end{tabular} \\ \midrule
Walmart-Amazon &
  \begin{tabular}[c]{@{}c@{}}66.30\\ (-)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}52.32\\ (34.11)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}42.70\\ (31.18)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}51.56\\ (-)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}45.16\\ (75.34)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}46.13\\ (73.83)\end{tabular} &
  25.89\% \\ \midrule
DBLP-Scholar &
  \begin{tabular}[c]{@{}c@{}}32.53\\ (-)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}37.23\\ (90.03)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}35.98\\ (85.14)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}29.17\\ (-)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}27.98\\ (81.96)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}29.95\\ (77.82)\end{tabular} &
  94.09\% \\ \midrule
WDC Products &
  \begin{tabular}[c]{@{}c@{}}44.75\\ (-)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}24.18\\ (78.76)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}23.20\\ (70.66)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}33.39\\ (-)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}28.43\\ (85.11)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}30.69\\ (83.94)\end{tabular} &
  77.36\% \\ \bottomrule
\end{tabular}%
}
\end{table}
